UniCL: A Universal Contrastive Learning Framework for Large Time Series Models

Time-series analysis plays a pivotal role across a range of critical applications, from finance to healthcare, which involves various tasks, such as forecasting and classification. To handle the inherent complexities of time-series data, such as high dimensionality and noise, traditional supervised learning methods first annotate extensive labels for time-series data in each task, which is very costly and impractical in real-world applications. In contrast, pre-trained foundation models offer a promising alternative by leveraging unlabeled data to capture general time series patterns, which can then be fine-tuned for specific tasks. However, existing approaches to pre-training such models typically suffer from high-bias and low-generality issues due to the use of predefined and rigid augmentation operations and domain-specific data training. To overcome these limitations, this paper introduces UniCL, a universal and scalable contrastive learning framework designed for pretraining time-series foundation models across cross-domain datasets. Specifically, we propose a unified and trainable time-series augmentation operation to generate pattern-preserved, diverse, and low-bias time-series data by leveraging spectral information. Besides, we introduce a scalable augmentation algorithm capable of handling datasets with varying lengths, facilitating cross-domain pretraining. Extensive experiments on two benchmark datasets across eleven domains validate the effectiveness of UniCL, demonstrating its high generalization on time-series analysis across various fields.

==> section/sec-backup.tex <==
\section{Backup}

\subsection{Time-series augmentation contrasting}
In real-world applications, the scarcity of well-annotated time-series data prompts researchers to integrate contrastive learning to acquire high-quality time-series representations, which can be easily transferred to downstream tasks. In this paper, the terms 'representation' and 'embedding' are used interchangeably to denote the learned vector representations of time-series.

\textbf{\textit{1) Pre-train time-series representation with contrastive learning:}} Contrastive learning aims to learn an encoder function $f_{\boldsymbol{\theta}}(\cdot)$ by contrasting between positive and negative samples, and augmentation contrast is one of the most widely used contrastive frameworks~\cite{zhang2023ssl4ts}. Specifically, given a mini-batch of input time-series $\mathcal{X}=\{\mathbf{{x}}_k\}_{k=1}^{n}$ and a family of augmentations $\mathcal{T}$, data augmentation operations sampled from $\mathcal{T}$ are applied to create two set of positive views $\tilde{\mathcal{X}}=\{\tilde{\mathbf{{x}}}_k\}_{k=1}^{n}$ and $\bar{\mathcal{X}}=\{\bar{\mathbf{{x}}}_k\}_{k=1}^{n}$. The positive pairs $(\tilde{\mathbf{{x}}}_{k}, \bar{\mathbf{{x}}}_{k})_{k=1}^{n}$ are expected to retain crucial temporal information, and the corresponding representations, $\tilde{\boldsymbol{z}}_k = f_{\boldsymbol{\theta}}(\tilde{\mathbf{{x}}}_{k})$ and $\bar{\boldsymbol{z}}_k = f_{\boldsymbol{\theta}}(\bar{\mathbf{{x}}}_{k})$, should exhibit proximity within the embedding space. The negative views of $\mathbf{{x}}_k$, denoted as $Neg(\mathbf{{x}}_k)$, comprise a set of time-series that exhibit dissimilarity to $\mathbf{{x}}_k$. To promote proximal representations of positive pairs while ensuring distant representations of negative set, the encoder $f_{\boldsymbol{\theta}}$ is optimized by the contrastive loss $l_{cl}(\cdot)$:

\begin{equation}
	\boldsymbol{\theta}^* = \arg \min_{\boldsymbol{\theta}} \frac{1}{n}\sum_{k=1}^{n}l_{cl}(f_{\boldsymbol{\theta}},\tilde{\mathbf{{x}}}_k,\bar{\mathbf{{x}}}_k,Neg(\mathbf{{x}}_k))
\end{equation}

\noindent One widely used $l_{cl}$~\cite{chen2020simple} is defined as:

\begin{equation}
	l_{cl} = - \log \frac{\exp(\text{sim}(\tilde{\boldsymbol{z}}_k, \bar{\boldsymbol{z}}_k)/\tau)}{\sum_{i=1}^{2n} \mathbbm{1}_{[i\neq k]} \exp(\text{sim}(\tilde{\boldsymbol{z}}_k, \tilde{\boldsymbol{z}}_i)/\tau)+\exp(\text{sim}(\tilde{\boldsymbol{z}}_k, \bar{\boldsymbol{z}}_i)/\tau)}
\end{equation}

%To encourage closer representations of positive pairs in a high-dimensional space and ensure distant representations of negative pairs, a widely used objective function~\cite{chen2020simple} in this framework is:

%\begin{equation}
%	\mathcal{L} = - \log \frac{\exp(\text{sim}(z_1, z_2)/\tau)}{\sum_{k=1}^{2N} \mathbbm{1}_{[k\neq i]} \exp(\text{sim}(z_1, z_k)/\tau)}
%\end{equation}

\noindent Where $\tau$ represents the temperature parameter, and $sim(\cdot)$ denotes the similarity function. 


\textbf{\textit{2) Fine-tuning time-series representations on downstream tasks:}} Given a pre-trained encoder $f_{\boldsymbol{\theta^*}}$ and an annotated task dataset $\mathcal{D}=\{\mathcal{X},\mathcal{Y}\}$, the objective is to train a decoder $q_{\boldsymbol{\phi}}$ by minimizing the task-specific loss $l_{\text{task}}$:

\begin{equation}
	\boldsymbol{\phi}^* = \arg \min_{\boldsymbol{\phi}}l_{\text{task}}(f_{\boldsymbol{\theta^*}},\mathcal{D},q_{\boldsymbol{\phi}})
\end{equation}

It is worth noting that the pre-trained encoder can also be fine-tuned during this stage.

Existing contrastive learning approaches mainly differ in positive view generation, and can be classified into two types: context-based and augmentation-based. Context-based approaches~\cite{yue2022ts2vec,tonekaboni2021unsupervised,kiyasseh2021clocs} generally advocate contextual consistency, considering sub-series with close temporal relationships as positive views. For example, TS2Vec~\cite{yue2022ts2vec} randomly selects two overlapping time segments $\mathbf{{x}}_{[a1:b1]}$ and $\mathbf{{x}}_{[a2:b2]}$ such that $0 < a1\leq a2 \leq b1\leq b2 \leq T$, and treats the overlapping segments as positive pairs. Other researchers~\cite{tonekaboni2021unsupervised,kiyasseh2021clocs} opt for temporal neighborhood sub-series as positive pairs. However, akin to masked modeling, context-based methods are reliant on observed data and may perform poorly on unseen data, thereby failing to address the issue of data-scarcity.



Instead, augmentation-based methods can generate diverse time-series based on observed data, improving the generality of the model. Current augmentation-based methods utilize pre-defined data augmentation operation to generate positive views. These methods include jittering~\cite{yeh2023toward,ijcai2021-324,raghu2023sequential}, scaling~\cite{woo2022cost}, permutation~\cite{meng2023mhccl,poppelbaum2022contrastive}, magnitude warping~\cite{fan2020self}, masking~\cite{yue2022ts2vec,wang2024contrast}, pooling~\cite{liang2023contrastive}, etc. Some researchers~\cite{zhang2022self,liu2024timesurl} also apply perturbation in the frequency domain. To further improve the generality of the model, CLUDA~\cite{ozyurt2023contrastive} adopts a composition of operations to generate positive views. However, relying on pre-defined operations entails a dependence on expert knowledge~\cite{ma2023survey} and is susceptible to inductive bias~\cite{saunshi2019theoretical}. Some researchers~\cite{ijcai2021-324,yue2022ts2vec} have observed that data augmentation is data-dependent, and inappropriate augmentations can lead to poorly learned representations. A more recent study~\cite{luo2023time} employs meta-learning to select augmentation operations adaptively  based on criteria of fidelity and variety. Nonetheless, they still rely on a pre-defined set of augmentations.


\subsection{Time-series analysis with LLMs}

Recently, there has been a surge of interests in time-series analysis leveraging Language Foundation Models (LFM), including BERT~\cite{sun2023test}, T5~\cite{ansari2024chronos}, LLaMA~\cite{gruver2023llmtime, jin2024time, jin2023time, rasul2023lag, liu2024autotimes}, and GPT~\cite{gruver2023llmtime, jin2024time, liu2024lstprompt, liu2024taming, pan2024textbf, bian2024multi, liu2024autotimes, liu2024large,liu2024can, chen2023gatgpt, liu2023unitime, cao2024tempo, chang2023llm4ts, sun2023test, zhou2023onefitsall}. In this paper, we only focus on decoder-only LLMs, \textit{i.e.,} GPT and LLaMA. Given a sequence of token embeddings $\boldsymbol{T}=\{\boldsymbol{t}_1, \boldsymbol{t}_2,\cdots,\boldsymbol{t}_N\}$, where $\boldsymbol{t}\in\mathbb{R}^{D}$ and $D$ is the dimension of input embedding, the LLM $f_{\boldsymbol{\theta}}$, composed of $L$ stacked transformer layers, adeptly captures the inherent temporal dependencies among input tokens. It generates token-wise representations $\boldsymbol{F}\in\mathbb{R}^{N\times D}$, matching the dimensions of $\boldsymbol{T}$, which can be effectively leveraged for downstream tasks. Typically, time-series analysis leveraging LLMs comprises three parts, namely, tokenization of the input time-series, generation of token embeddings, and fine-tuning of the LLM.

\textbf{\textit{1) Tokenization of the input time-series: }} Given input series $\mathbf{{x}}\in\mathbb{R}^T$, the transformer exhibits $O(T^2)$ complexity in both time and space. Moreover, each time point $\mathbf{{x}}_i$ can only carry very sparse semantic~\cite{cheng2023timemae}, and is prone to noise. Tokenization of time-series involves aggregating time points into tokens, demonstrated to be both efficient and effective. The most widely used method is patching~\cite{Yuqietal-2023-PatchTST}, where $\mathbf{{x}}$ is divided into overlapped or non-overlapped patches. Let the patch length be $P$ and the stride be $S$. Then, the tokenizer will generate a sequence of patches $\boldsymbol{X}_p \in \mathbb{R}^{N \times P}$  where  $N$ is the number of patches, $N = \left\lfloor \frac{(L-P)}{S} \right\rfloor + 2$. Except for patching, other tokenization methods include binning~\cite{ansari2024chronos} and stringify~\cite{gruver2023llmtime}. CHRONOS~\cite{ansari2024chronos} performs tokenization by discretizing time-series into discrete bins through simple scaling and quantization of real values. LLMTIME~\cite{gruver2023llmtime} encodes time-series as a string of numerical digits, with each digit separated by spaces to conform to the requirements of the off-the-shelf NLP tokenizer. Recently, some studies have utilized feature engineering techniques (e.g., decomposition~\cite{cao2024tempo,pan2024textbf}, lag features~\cite{rasul2023lag}) prior to the tokenization process to enable LLM better capture the intrinsic dynamics. \jiawei{cons}However, relying solely on tokenization is insufficient for building a comprehensive time-series large model, and feature engineering necessitates prior knowledge, which is not suitable for large-scale pre-training.


\textbf{\textit{2) Generation of token embeddings: }} To align with the intrinsic dimension $D$ of LLMs, the input embedding layer map the sequence of tokens $\boldsymbol{X}_p$ to the embedding space $\boldsymbol{T}\in\mathbb{R}^{N\times D}$. In NLP, such mapping is achieved via a word embedding dictionary $\boldsymbol{M}\in\mathbb{R}^{\left|A\right|\times D}$, where $\left|A\right|$ is the size of the alphabet. To bridge the modality gap between language and time-series data, various approaches have been explored to align their embedding spaces. These include techniques such as knowledge distillation~\cite{liu2024taming}, score-matching function~\cite{pan2024textbf}, and contrastive learning~\cite{sun2023test}. For instance,  TEST~\cite{sun2023test} trains a general embedding layer, comprising a $10$-layer convolutional block, using instance-wise, feature-wise, and text-prototype-aligned contrasting to align the time series embedding with the text embedding.  However, TEST relies on a predefined data augmentation strategy for generating positive pairs, potentially introducing inductive bias.


\textbf{\textit{3) Fine-tuning of the LLM: }} The decoder-only LLM $f_{\boldsymbol{\theta}}$ takes token embeddings $\boldsymbol{T}$ as input and generates token-wise representations $\boldsymbol{F}$, which are applicable for downstream tasks. \jiawei{1 finetune}A line of research~\cite{zhou2023onefitsall, chang2023llm4ts, chen2023gatgpt, liu2024lstprompt, liu2024can, liu2024autotimes, xue2023promptcast} applies Parameter-Efficient Fine-Tuning (PEFT), that fine-tuning a small subset of parameters to adapt pre-trained LLMs to down-stream tasks. For instance, GPT4TS~\cite{zhou2023onefitsall} and GATGPT~\cite{chen2023gatgpt} freeze the self-attention and \textit{Feedforward} layers, while adjusting the positional embeddings and \textit{LayerNorm} layers of pre-trained GPT-2. LLM4TS~\cite{chang2023llm4ts} also applies Low-Rank Adaptation (LoRA) to the self-attention layer. \jiawei{Cons}However, these approaches only adjust a few parameters of LLMs, necessitating the use of separate models for each dataset, thereby limiting their generality. \jiawei{2 prompting}Another PEFT technique, prompting, involves concatenating additional tokens with the original input tokens to guide the LLMs in generating contextually relevant outputs. Some researchers~\cite{liu2024lstprompt, liu2024can, liu2024autotimes, xue2023promptcast} incorporate domain information (e.g., traffic, weather) and frequency (e.g., hour, day) into template-based descriptions, embedding them as tokens using a text tokenizer. LSTPrompt~\cite{liu2024lstprompt} employs a \textit{Chain-of-Thought} approach to guide the LLM in making predictions in a zero-shot manner.  Instead of concatenating prompts, AutoTimes~\cite{liu2024autotimes} blends the prompts embedding and time series embedding within the same time segment to exploit the inherent transition of LLM. \jiawei{Cons}However, these approaches require domain-specific knowledge and task-specific information, limiting their generality to broader applications. One potential solution is to utilize soft prompts~\cite{cao2024tempo, sun2023test, sun2023test}, which can be randomly initialized and trained, thereby offering greater flexibility. 

%\jiawei{2 tokenizor} \jiawei{Instead of adjusting the parameters of LLM, another line of research~\cite{cao2024tempo, ansari2024chronos, gruver2023llmtime} preprocess the input numerical values in order to facilitate the understanding of LLM. For example, LLMTIME~\cite{gruver2023llmtime} encodes time series data as a string of numerical digits, with each digit separated by spaces to conform to the requirements of the off-the-shelf tokenizer. CHRONOS~\cite{ansari2024chronos} performs tokenization on time series data by discretizing them into discrete bins through simple scaling and quantization of real values. Lag-Llama~\cite{rasul2023lag} generates lag features as covariates from quarterly, monthly, weekly, daily, and hourly lag indices. TEMPO~\cite{cao2024tempo} and $S^2IP-LLM$ utilize seasonal and trend decomposition from STL~\cite{cleveland1990stl} to decompose the input time series to enable LLM better capture the intrinsic dynamics. \jiawei{cons}However, relying solely on input transformations is insufficient to achieve a unified time-series large model.}

More recently, there have been some efforts~\cite{liu2023unitime,rasul2023lag,bian2024multi,garza2023timegpt} directed towards developing universal time-series forecasting models, aiming to address forecasting tasks across various domains. These models utilize self-supervised training on datasets from various domains and directly employ future prediction as pretext tasks. Specifically, UniTime~\cite{liu2023unitime} frames its pretext task as predicting the subsequent values, whereas aLLM4TS~\cite{bian2024multi} formulates the pretext task as the next patch prediction. TimeGPT~\cite{garza2023timegpt} and Lag-Llama~\cite{rasul2023lag} utilize probabilistic forecasting, estimating model uncertainty around predictions. These approaches prioritize the predictive ability over generality and lack the instance-wise representation of time series, which is crucial for the classification task. \jiawei{lack UniTS}


%\subsection{Problem Definition}
%%Given an input LLM as the backbone, the object is to re-train this LLM on cross-domain time-series datasets $\mathcal{D}=\{D_i|i=1,...,n\}$, in order to obtain a unified time-series foundation model $f_{\boldsymbol{\theta}}$.
%In this work, we focus on the problem of pre-training a unified time-series foundation model.\jiawei{need to discuss, UniTS}
%
%\begin{definition}\textbf{(Unified time-series foundation model).}
%	%Given an input time-series  $\boldsymbol{X}\in \mathbb{R}^{T\times F}$, where $T$ is the sequence length, and $F$ is the dimension of features, the object is to learn an encoder $f_{\boldsymbol{\theta}}(\boldsymbol{X})$ that maps the input time-series to a representation matrix $\boldsymbol{Z}\in \mathbb{R}^{T\times D}$, where $\boldsymbol{\theta}$ is the learnable parameters, and $D$ ($D > F$) is the dimension of representation.
%	A unified time-series foundation model $f_{\boldsymbol{\theta}}$ refers to a pre-trained deep learning model that serves as a fundamental building block for a wide range of time-series tasks.  Given an input uni-variate time-series $x\in\mathbb{R}^{T}$, the time-series tokenizer converts it into a token matrix $X_{\text{token}}\in\mathbb{R}^{P\times D}$, where $P$ ($P < T$) denotes the number of tokens and $D$ represents the hidden dimension of the foundation model. Utilizing $X_{\text{token}}$ as input, the foundation model produces a representation matrix $Z\in\mathbb{R}^{P\times D}$.
%\end{definition}
%
%The model $f_{\boldsymbol{\theta}}$ is trained on large-scale datasets and learn rich, temporal representations of time-series. Due to its versatility and effectiveness, foundation model can be fine-tuned or adapted to specific downstream tasks with relatively little task-specific data or even without data.


\clearpage



==> section/sec-data_augmentation_module.tex <==
\section{Framework Overview}\label{sec:framework}


\subsection{Motivational observation of bias in embedding}



As discussed in Sec.1, existing pre-defined time-series augmentation methods introduce an \textbf{\textit{inductive bias}} into representation learning amidst augmentation contrast. We present our key motivational observation: \textit{the bias in time-series embedding correlates positively with the \textbf{spectral distance} between raw and augmented series.} To illustrate, we first quantify the bias introduced by the data augmentation $\mathcal{T}(\cdot)$ as follows, in line with previous work~\cite{zhang2022costa}. Denote the $i$-th input sample as $\boldsymbol{x_i}$ and its corresponding augmentation set as $\tilde{\mathcal{X}_i}$. Each augmented series $\boldsymbol{\tilde{x}}_i^{(k)}\in \tilde{\mathcal{X}_i}$ is generated through the stochastic transformation $\mathcal{T}(\boldsymbol{x_i})$. Let $\tilde{\mathcal{T}}(\boldsymbol{x_i})$ symbolize the transformation distribution of $\boldsymbol{x_i}$, while $f(\cdot)$ represents the encoder function. Then,


\begin{equation}
	\label{bias}
	\begin{aligned}
		\text{Bias}(\mathcal{T}(\boldsymbol{x_i})) &= 
		\Big \lVert 
		\mathbb{E}_{
			\tilde{\boldsymbol{x_i}}
			\sim
			\tilde{\mathcal{T}} 
			(\boldsymbol{x_i} )
		}
		\big (f (\tilde{\boldsymbol{x}}_i)\big )-f(\boldsymbol{x_i})
		\Big \rVert_2 \\
		& \approx \Big \lVert 
		\frac{1}{
			\big| \tilde{\mathcal{X}_i} \big|
		} \sum_{k=1}^{
			\small | \tilde{\mathcal{X}_i} \small |
		}  
		f (\boldsymbol{\tilde{x}}_i^{(k)})-f(\boldsymbol{x_i})
		\Big \rVert_2
	\end{aligned}
\end{equation}

\noindent Given $MSE(\cdot)$, $fft(\cdot)$, and $Amp(\cdot)$ representing mean-squared error, Fast Fourier Transform (FFT), and amplitude calculation respectively, the \textit{spectral distance} between $\boldsymbol{x_i}$ and $\tilde{\boldsymbol{x}}_i$ is defined as:

\begin{equation}
	\label{spectraldistance}
	SD(\boldsymbol{x_i},\tilde{\boldsymbol{x}_i}) = MSE\big (Amp(fft(\boldsymbol{x_i})), Amp(fft(\tilde{\boldsymbol{x}}_i))\big )
\end{equation}

We employ the representative and state-of-the-art contrastive learning method TS2Vec~\cite{yue2022ts2vec} to test 6 pre-defined augmentation methods on 23 selected multivariate datasets from the UEA Time Series Classification Archive~\cite{bagnall2018uea} and report the average bias and spectral distance. For each dataset, we train the TS2Vec encoder with the same configuration as the original paper but varying the augmentation method. These methods encompass jittering, scaling, time warping, pooling, permutation, and cut out, each offering diverse variants achieved by adjusting hyperparameters (e.g., the standard deviation of jittering). The output layer of the encoder has two dimensions to facilitate visualization. Following, we generate $\big| \tilde{\mathcal{X}_i} \big| = 500$ augmented samples randomly for each sample, and compute the bias and the average spectral distance using equations~\ref{bias} and~\ref{spectraldistance}, respectively. Figure~\ref{motivational}(a) illustrates a positive correlation between the bias and the average spectral distance of augmented and raw series. Meanwhile, Figure~\ref{motivational}(b) demonstrates that greater bias in the embeddings results in reduced performance in downstream classification tasks. This observation motivates the need for time-series augmentation methods to control the spectral distance between augmented and raw time-series. As depicted in Figure~\ref{motivational}(c,d), within contrastive learning, a significant bias may hinder the effectiveness of separating augmented embeddings across different instances (\textit{i.e.}, $f(\boldsymbol{\tilde{x}}_i^{(k)}),f(\boldsymbol{\tilde{x}}_j^{(k)})$, where $i\neq j$), thus limiting the discriminative power of learned embeddings (\textit{i.e.}, $f(\boldsymbol{x}_i^{(k)}),f(\boldsymbol{x}_j^{(k)})$) for downstream tasks~\cite{zhang2022costa}. 


\begin{figure}[t]
	\begin{minipage}[t]{0.5\linewidth}
		\centering
		\includegraphics[width=1\textwidth]{figures/3.1(a)}
		\captionsetup{skip=0pt,font={small,stretch=0.9}}
		\caption*{(a) Spectral Distance and Bias}
	\end{minipage}%
	\begin{minipage}[t]{0.5\linewidth}
		\centering
		\includegraphics[width=1\textwidth]{figures/3.1(b)}
		\captionsetup{skip=0pt,font={small,stretch=0.9}}
		\caption*{(b) Bias and accuracy}
	\end{minipage}
	\begin{minipage}[t]{0.5\linewidth}
		\centering
		\includegraphics[width=1\textwidth]{figures/3.1(c)}
		\captionsetup{skip=0pt,font={small,stretch=0.9}}
		\caption*{(c) High-bias embedding}
	\end{minipage}%
	\begin{minipage}[t]{0.5\linewidth}
		\centering
		\includegraphics[width=1\textwidth]{figures/3.1(d)}
		\captionsetup{skip=0pt,font={small,stretch=0.9}}
		\caption*{(d) Low-bias embedding}
	\end{minipage}
	\captionsetup{skip=3pt}
	\captionsetup{justification=justified,singlelinecheck=false,font={small,stretch=0.9}}
	\caption{The bias observation of six pre-defined augmentation methods and each has eight variants. Fig. 1a illustrates the relationship between the average spectral distance of augmented and raw series and the average bias of learned embeddings. The y-axis represents bias, while the x-axis denotes the average spectral distance. Fig. 1b demonstrates the impact of embedding bias on downstream classification task. Here, the y-axis indicates the average accuracy, and the x-axis represents bias. Fig. 1c and Fig. 1d visualize the high-bias and low-bias of the embedding. }
	\label{motivational}
\end{figure}
\vspace{-0.1cm}


==> section/sec-related_work.tex <==
\section{Related work}\label{sec:related_work}
% $S^2IP-LLM$ considers existing text-token embeddings as prompt candidates and retrieves top-k prompts as prefix-prompt based on cosine similarity with time series embeddings.
\noindent\textbf{Contrastive learning.} 


\noindent\textbf{Time-series with language foundation models.} Recently, there has been a surge of interests in time-series analysis leveraging language foundation models, including BERT~\cite{sun2023test}, T5~\cite{ansari2024chronos}, LLaMA~\cite{gruver2023llmtime, jin2024time, jin2023time, rasul2023lag, liu2024autotimes}, and GPT~\cite{gruver2023llmtime, jin2024time, liu2024lstprompt, liu2024taming, pan2024textbf, bian2024multi, liu2024autotimes, liu2024large,liu2024can, chen2023gatgpt, liu2023unitime, cao2024tempo, chang2023llm4ts, sun2023test, zhou2023onefitsall}. 
\jiawei{1}A line of research~\cite{zhou2023onefitsall, chang2023llm4ts, chen2023gatgpt, liu2024lstprompt, liu2024can, liu2024autotimes, xue2023promptcast} applies Parameter-Efficient Fine-Tuning (PEFT), that fine-tuning a small subset of parameters to adapt pre-trained LLMs to down-stream tasks. For instance, GPT4TS~\cite{zhou2023onefitsall} and GATGPT~\cite{chen2023gatgpt} freeze the self-attention and \textit{Feedforward} layers, while adjusting the positional embeddings and \textit{LayerNorm} layers of pre-trained GPT-2. LLM4TS~\cite{chang2023llm4ts} also applies Low-Rank Adaptation (LoRA) to the self-attention layer. \jiawei{Cons}However, these approaches only adjust a few parameters of LLMs, necessitating the use of separate models for each dataset, thereby limiting their generality. \jiawei{2}Another PEFT technique, prompting, involves concatenating additional tokens with the original input tokens to guide the LLMs in generating contextually relevant outputs. Some researchers~\cite{liu2024lstprompt, liu2024can, liu2024autotimes, xue2023promptcast} incorporate domain information (e.g., traffic, weather) and frequency (e.g., hour, day) into template-based descriptions, embedding them as tokens using a text tokenizer. LSTPrompt~\cite{liu2024lstprompt} employs a \textit{Chain-of-Thought} approach to guide the LLM in making predictions in a zero-shot manner.  Instead of concatenating prompts, AutoTimes~\cite{liu2024autotimes} blends the prompts embedding and time series embedding within the same time segment to exploit the inherent transition of LLM. \jiawei{Cons}However, these approaches require domain-specific knowledge and task-specific information, limiting their generality to broader applications. One potential solution is to utilize soft prompts~\cite{cao2024tempo, sun2023test, sun2023test}, which can be randomly initialized and trained, thereby offering greater flexibility. \jiawei{2}Instead of adjusting the parameters of LLM, another line of research~\cite{cao2024tempo, ansari2024chronos, gruver2023llmtime} preprocess the input numerical values in order to facilitate the understanding of LLM. For example, LLMTIME~\cite{gruver2023llmtime} encodes time series data as a string of numerical digits, with each digit separated by spaces to conform to the requirements of the off-the-shelf tokenizer. CHRONOS~\cite{ansari2024chronos} performs tokenization on time series data by discretizing them into discrete bins through simple scaling and quantization of real values. Lag-Llama~\cite{rasul2023lag} generates lag features as covariates from quarterly, monthly, weekly, daily, and hourly lag indices. TEMPO~\cite{cao2024tempo} and $S^2IP-LLM$ utilize seasonal and trend decomposition from STL~\cite{cleveland1990stl} to decompose the input time series to enable LLM better capture the intrinsic dynamics. \jiawei{cons}However, relying solely on input transformations is insufficient to achieve a unified time-series large model. 

More recently, there have been some efforts directed towards developing time-series foundation models. TEST~\cite{sun2023test} trains a universal input encoder, comprising a $10$-layer convolutional block, using instance-wise, feature-wise, and text-prototype-aligned contrasting to align the time series embedding with the text embedding. However, TEST utilizes a pre-defined data augmentation strategy to generate positive pairs, which may introduce inductive bias. UniTime~\cite{liu2023unitime}, Lag-Llama~\cite{rasul2023lag}, aLLM4TS~\cite{bian2024multi}, and TimeGPT~\cite{garza2023timegpt} are proposed as universal forecasting models, aiming to address time-series forecasting tasks across various domains. These models utilize self-supervised training on datasets from various domains and directly employ future prediction as pretext tasks. Specifically, UniTime~\cite{liu2023unitime} frames its pretext task as predicting the subsequent values, whereas aLLM4TS~\cite{bian2024multi} formulates the pretext task as the next patch prediction. TimeGPT~\cite{garza2023timegpt} and Lag-Llama~\cite{rasul2023lag} utilize probabilistic forecasting, estimating model uncertainty around predictions. These approaches prioritize the predictive ability over generality and lack the instance-wise representation of time series, which is crucial for the classification task.


% Chronos trains from scratch (probabilistic) liu2024lstprompt is prompt based liu2024taming 

